DualMS: Implicit Dual-Channel Minimal Surface Optimization for Heat Exchanger Design

Heat exchangers are critical components in a wide range of engineering applications, from energy systems to chemical processing, where efficient thermal management is essential. The design objectives for heat exchangers include maximizing the heat exchange rate while minimizing the pressure drop, requiring both a large interface area and a smooth internal structure. State-of-the-art designs, such as triply periodic minimal surfaces (TPMS), have proven effective in optimizing heat exchange efficiency. However, TPMS designs are constrained by predefined mathematical equations, limiting their adaptability to freeform boundary shapes. Additionally, TPMS structures do not inherently control flow directions, which can lead to flow stagnation and undesirable pressure drops. This paper presents DualMS, a novel computational framework for optimizing dual-channel minimal surfaces specifically for heat exchanger designs in freeform shapes. To the best of our knowledge, this is the first attempt to directly optimize minimal surfaces for two-fluid heat exchangers, rather than relying on TPMS. Our approach formulates the heat exchange maximization problem as a constrained connected maximum cut problem on a graph, with flow constraints guiding the optimization process. To address undesirable pressure drops, we model the minimal surface as a classification boundary separating the two fluids, incorporating an additional regularization term for area minimization. We employ a neural network that maps spatial points to binary flow types, enabling it to classify flow skeletons and automatically determine the surface boundary. DualMS demonstrates greater flexibility in surface topology compared to TPMS and achieves superior thermal performance, with lower pressure drops while maintaining a similar heat exchange rate under the same material cost.

==> tables/table-scalability.tex <==

\begin{table}[t]
\renewcommand{\arraystretch}{1}
\centering
\caption{ 
Program running time of each step (Second).
$Ori$ is the time of orientation determination of $M^*$.
$Pre$ is the time of Pre-processing.
$Ini$ is the time of initialization of cutting planes.
$MCTS$ is the time of Monte Carlo Tree Search.
$Pos$ is the time of Post-processing of generating AM positional blocks.
$T$ is the total running time (Minute).
}
\begin{tabular}{m{1.8cm}<{\centering}| m{0.65cm}<{\centering}  m{0.5cm}<{\centering} m{0.5cm}<{\centering} m{0.7cm}<{\centering} m{0.6cm}<{\centering} |m{0.8cm}<{\centering} }
\hline
{\#Facets} 
& \centering{$Ori$} 
& \centering{$Pre$}
& \centering{$Ini$}
& \centering{$MCTS$} 
& \centering{$Pos$} 
& {$T$} \\
\hline
%\rule{0pt}{15pt}
{\hspace*{-2pt}(a) \hspace*{2pt}3006}     &{99} &{12} &{10} &{58} &{1} &{3.0} \\
\hline
{\hspace*{-2pt}(b) \hspace*{2pt}6046}     &{121} &{13} &{17} &{101} &{2} &{4.2} \\
\hline
{(c) 12574}     &{172} &{16} &{30} &{229} &{5} &{7.5} \\
\hline
{(d) 25270}     &{253} &{20} &{59} &{285} &{9} &{10.4} \\
\hline
{(e) 50302}     &{429} &{29} &{\hspace*{-1pt}145} &{600} &{23} &{20.4} \\
\hline
\end{tabular}
\label{table:scalability}
\end{table}


==> tables/table-statistics.tex <==

\begin{table}[t]
\renewcommand{\arraystretch}{1.0}
\centering
\caption{Statistics of the models shown in the paper. 
$H$ represents the height of $M^*$ after its setup is determined.
$R_V$ is the volume ratio of $V^I$ to $M^*$.
$A$ is the ratio of the minimum Z-value of the additive interfaces to the height of $M$.
$\#P_S$ and $\#P_A$ indicates the number of SM and AM inaccessible points, respectively.
$R_I$ is the volume ratio of $V^{I'}$ to $M^*$ after initial surface evolution.
$\#C_b$ and $\#C_a$ are the number of clipping planes before and after MCTS, respectively.
$R_F$ is the final volume ratio of determined $V^{I*}$ to $M^*$.
$\#B_S$ and $\#B_A$ are the number of SM/AM positional blocks.
}
\begin{tabular}{m{1.2cm}<{\centering}  m{0.2cm}<{\centering}| m{0.3cm}<{\centering} m{0.4cm}<{\centering}  m{0.2cm}<{\centering} m{0.2cm}<{\centering}| m{0.35cm}<{\centering} m{0.2cm}<{\centering}| m{0.2cm}<{\centering} m{0.39cm}<{\centering}| m{0.2cm}<{\centering} m{0.2cm}<{\centering}} 
\hline
\multicolumn{2}{c|}{}&\multicolumn{4}{c|}{Sec. 4.2}&\multicolumn{2}{c|}{Sec. 4.3}&\multicolumn{2}{c|}{Sec. 4.4}&\multicolumn{2}{c}{Sec. 5}\\
\hline
{Model} 
&{\hspace*{-2pt}$H$} 
&{\hspace*{3pt}$R_V$} 
&{\hspace*{3pt}$A$}
&{\hspace*{-3pt}$\#P_S$} 
&{\hspace*{-5pt}$\#P_A$}
&{$R_I$} 
&{\hspace*{-4pt}$\#C_b$}
&{\hspace*{-2pt}$\#C_a$}
&{\hspace*{2pt}$R_F$} 
&{\hspace*{-3pt}$\#B_S$} 
&{\hspace*{-3pt}$\#B_A$} 
\\
\hline
{Bearing}     &{\hspace*{-3pt}34} &{0.98} &{0.51} &{0} &{\hspace*{-3pt}5} &{0.81} &{2} &{2} &{\hspace*{-2pt}\textbf{0.90}} &{5} &{2}\\
\hline
{Hand}        &{\hspace*{-3pt}77} &{0.91} &{0.31} &{\hspace*{-2pt}23} &{\hspace*{-5pt}167} &{0.70} &{1} &{2} &{\hspace*{-2pt}\textbf{0.80}} &{5} &{\hspace*{-1pt}3}\\
\hline
{Coral}       &{\hspace*{-3pt}53} &{0.92} &{0.41} &{2} &{\hspace*{-3pt}57} &{0.40} &{\hspace*{-2pt}2} &{\hspace*{-2pt}6} &{\hspace*{-2pt}\textbf{0.62}} &{5} &{\hspace*{-1pt}5}\\
\hline
{Bracket}     &{\hspace*{-3pt}57} &{0.55} &{1.00} &{5} &{\hspace*{-3pt}0} &{0.42} &{1} &{3} &{\hspace*{-2pt}\textbf{0.51}} &{5} &{4}\\
\hline
{Holder}      &{\hspace*{-3pt}58} &{0.77} &{1.00} &{8} &{\hspace*{-3pt}0} &{0.31} &{1} &{2} &{\hspace*{-2pt}\textbf{0.37}} &{5} &{1}\\
\hline
{Opener}      &{\hspace*{-5pt}191} &{0.54} &{0.94} &{7} &{\hspace*{-3pt}0} &{0.35} &{3} &{3} &{\hspace*{-2pt}\textbf{0.52}} &{\hspace*{-1pt}5} &{3}\\
\hline
{Impeller}      &{\hspace*{-5pt}35} &{0.92} &{1.00} &{48} &{\hspace*{-3pt}0} &{0.62} &{1} &{1} &{\hspace*{-2pt}\textbf{0.74}} &{\hspace*{-1pt}9} &{7}\\
\hline
{Sculpture}      &{\hspace*{-3pt}46} &{0.98} &{0.26} &{0} &{\hspace*{-3pt}3} &{0.65} &{4} &{5} &{\hspace*{-2pt}\textbf{0.69}} &{5} &{5}\\
\hline
{Prince}      &{\hspace*{-3pt}33} &{0.78} &{0.89} &{0} &{\hspace*{-3pt}0} &{0.46} &{2} &{2} &{\hspace*{-2pt}\textbf{0.75}} &{5} &{2}\\
\hline
{Cow}        &{\hspace*{-3pt}46} &{0.74} &{0.57} &{0} &{\hspace*{-3pt}0} &{0.62} &{1} &{1} &{\hspace*{-2pt}\textbf{0.73}} &{5} &{1}\\
\hline
{Swan}        &{\hspace*{-3pt}53} &{0.87} &{0.43} &{\hspace*{-2pt}21} &{\hspace*{-3pt}3} &{0.53} &{1} &{2} &{\hspace*{-2pt}\textbf{0.75}} &{6} &{2}\\
\hline
{Tree}        &{\hspace*{-3pt}55} &{0.93} &{0.49} &{\hspace*{-2pt}7} &{\hspace*{-3pt}0} &{0.81} &{7} &{12} &{\hspace*{-2pt}\textbf{0.85}} &{7} &{8}\\
\hline
%{Fertility}     &{90} &{0.21} &{3521} &{202} &{0.06} &{/} &{/} &{/} &{/} &{/}\\
%\hline
\end{tabular}
\label{table:data}
\end{table}

==> tables/table-time.tex <==

\begin{table}[t]
\renewcommand{\arraystretch}{1.0}
\centering
\caption{ 
Program running time of each step (second).
$Ori$ is the time to determine the setup of $M^*$.
$Pre$ is the time of Pre-processing.
$Ini$ represents the time of initialization of clipping planes.
$MCTS$ is the time of the Monte Carlo Tree Search.
$Pos$ represents the post-processing time for generating AM positional blocks.
$T$ is the total running time (minute).
}
\begin{tabular}{m{1.8cm}<{\centering}| m{0.65cm}<{\centering}  m{0.5cm}<{\centering} m{0.5cm}<{\centering} m{0.7cm}<{\centering} m{0.6cm}<{\centering} |m{0.8cm}<{\centering} }
\hline
{Model} 
& \centering{$Ori$} 
& \centering{$Pre$}
& \centering{$Ini$}
& \centering{$MCTS$} 
& \centering{$Pos$} 
& {$T$} \\
\hline
%\rule{0pt}{15pt}
{Bearing}     &{166} &{9} &{13} &{194} &{2} &{6.4} \\
\hline
{Hand}     &{215} &{37} &{22} &{527} &{5} &{13.4} \\
\hline
{Coral}     &{114} &{11} &{69} &{157} &{4} &{5.9} \\
\hline
{Bracket}     &{111} &{56} &{8} &{401} &{4} &{9.7} \\
\hline
{Holder}     &{92} &{18} &{10} &{220} &{5} &{5.8} \\
\hline
{Opener}     &{145} &{24} &{27} &{415} &{81} &{11.5} \\
\hline
{Impeller}     &{197} &{37} &{8} &{510} &{37} &{13.2} \\
\hline
{Sculpture}     &{195} &{17} &{38} &{240} &{6} &{8.3} \\
\hline
{Prince}     &{205} &{9} &{9} &{134} &{2} &{6.0} \\
\hline
{Cow}     &{63} &{6} &{2} &{81} &{1} &{2.6} \\
\hline
{Swan}     &{178} &{21} &{21} &{399} &{8} &{10.5} \\
\hline
{Tree}     &{157} &{17} &{52} &{88} &{8} &{5.4} \\
\hline
\end{tabular}
\label{table:runtime}
\end{table}

